Forecasting Clinical Risk from Textual Time Series: Structuring Narratives for Temporal AI in Healthcare

Clinical case reports encode temporal patient trajectories that are often underexploited by traditional machine learning methods relying on structured data. In this work, we introduce the forecasting problem from textual time series, where timestamped clinical findings -- extracted via an LLM-assisted annotation pipeline -- serve as the primary input for prediction. We systematically evaluate a diverse suite of models, including fine-tuned decoder-based large language models and encoder-based transformers, on tasks of event occurrence prediction, temporal ordering, and survival analysis. Our experiments reveal that encoder-based models consistently achieve higher F1 scores and superior temporal concordance for short- and long-horizon event forecasting, while fine-tuned masking approaches enhance ranking performance. In contrast, instruction-tuned decoder models demonstrate a relative advantage in survival analysis, especially in early prognosis settings. Our sensitivity analyses further demonstrate the importance of time ordering, which requires clinical time series construction, as compared to text ordering, the format of the text inputs that LLMs are classically trained on. This highlights the additional benefit that can be ascertained from time-ordered corpora, with implications for temporal tasks in the era of widespread LLM use.

==> Tables/clean_forecasting_DS.tex <==
\begin{table}[htbp]
%\footnotesize
\caption{Forecasting performance (event occurrence: F1 and correct event ordering: concordance-index) of the ensuing $k=8$ events. All models are trained/fine-tuned on time-ordered annotations from \texttt{DeepSeek-R1}. \textbf{Bold} values indicate best in category amongst all models.}
\label{tab:DS_forecasting_clean}
\label{apd:full_tables}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{\textit{T2S2} (\texttt{DeepSeek-R1})} & \multicolumn{2}{c}{\textit{sepsis-10}} & \multicolumn{2}{c}{\textit{sepsis-100}}\\
& F1(1h) & F1(1d) & F1(1w) & c-index & F1(1d) & c-index & F1(1d) & c-index\\
\midrule
\textbf{LLM-MLP head} &&&&&&&&\\
DS-L3.3 70B & \textbf{0.075} & 0.482 & \textbf{0.796} & \textbf{0.632} & \textbf{0.397} & \textbf{0.578} & \textbf{0.613} & 0.595 \\
\textbf{Prompting} &&&&&&&&\\
L3.3 70B few-shot & \textbf{0.095} & \textbf{0.380} & 0.652 & -- & \textbf{0.360} & -- & 0.452 & -- \\
\midrule
\textbf{Encoder-MLP head} &&&&&&&&\\
ModernBERT-base & \textbf{0.306} & \textbf{0.576} & \textbf{0.877} & \textbf{0.646} & 0.428 & \textbf{0.562} & 0.607 & \textbf{0.558} \\
\midrule
\textbf{Encoder-masking-fine-tuned} &&&&&&&&\\
ModernBERT-base & \textbf{0.186} & 0.449 & \textbf{0.697} & \textbf{0.672} & 0.325 & 0.576 & \textbf{0.503} & 0.613 \\
\midrule
\textbf{Encoder-masking-zeroshot} &&&&&&&&\\
ModernBERT-base & 0.169 & \textbf{0.468} & \textbf{0.804} & 0.496 & \textbf{0.358} & 0.501 & \textbf{0.511} & 0.499 \\
ModernBERT-large & 0.133 & 0.349 & 0.534 & 0.494 & 0.271 & 0.509 & 0.277 & 0.502 \\
\bottomrule
\end{tabular}
}
\end{table}


==> Tables/clean_forecasting_L33.tex <==
\begin{table}[!htbp]
%\footnotesize
\caption{Forecasting performance (event occurrence: F1 and correct event ordering: concordance-index) of the ensuing $k=8$ events. All models are trained/fine-tuned on time-ordered annotations from \texttt{Llama-3.3-70B}. \textbf{Bold} values indicate best in category amongst all models.}
\label{tab:L33_forecasting_clean}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{\textit{T2S2} (\texttt{Llama-3.3)}} & \multicolumn{2}{c}{\textit{sepsis-10}} & \multicolumn{2}{c}{\textit{sepsis-100}} \\
& F1(1h) & F1(1d) & F1(1w) & c-index & F1(1d) & c-index & F1(1d) & c-index \\
\midrule
\textbf{LLM-MLP head} &&&&&&&&\\
DS-L3.3 70B & 0.140 & 0.563 & 0.811 & \textbf{0.624} & \textbf{0.397} & \textbf{0.585} & \textbf{0.629} & \textbf{0.598} \\
\textbf{Prompting} &&&&&&&&\\
L3.3 70B few-shot ordinal & 0.064 & \textbf{0.460} & \textbf{0.729} & -- & 0.313 & -- & 0.480 & -- \\
\midrule
\textbf{Encoder-MLP head} &&&&&&&&\\
ModernBERT-base & 0.257 & \textbf{0.645} & \textbf{0.903} & 0.594 & 0.431 & \textbf{0.590} & \textbf{0.626} & 0.565 \\
\midrule
\textbf{Encoder-masking-fine-tuned} &&&&&&&&\\
ModernBERT-base & \textbf{0.139} & \textbf{0.489} & 0.700 & 0.632 & \textbf{0.334} & 0.595 & \textbf{0.478} & 0.612 \\
\midrule
\textbf{Encoder-masking-zeroshot} &&&&&&&&\\
ModernBERT-base & \textbf{0.132} & \textbf{0.525} & \textbf{0.840} & 0.556 & \textbf{0.352} & 0.503 & 0.511 & 0.501 \\

\bottomrule
\end{tabular}
}
\end{table}


==> Tables/textord_train_timeord_eval.tex <==
\begin{table*}[tb!]
%\footnotesize
\caption{Comparison of approaches by test-set forecasting performance of the ensuing $k=8$ events. \textbf{All models are trained/fine-tuned on text-ordered data. \textcolor{red}{For our own reference, 0.5 value means model is not learning at all}}}
\label{tab:results}
\small
\centering
\begin{tabular}{lcccccc}
\toprule
% & c-index & F1 ($0 < t \leq 24$) & F1 ($0 < t \leq 168$) & F1 ($0 < t \leq 8760$) \\
& \multicolumn{4}{c}{\textit{T2S2} (Llama 3.3)} & \multicolumn{2}{c}{sepsis-10}\\
& F1(1h) & F1(1d) & F1(1w) & c-index & F1(1d) & c-index\\
% & \multicolumn{3}{c}{i2m4} & \multicolumn{3}{c}{sepsis-10} & \multicolumn{3}{c}{sepsis-100} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% \textbf{Model} & Event & c-index & AULTC & Event & c-index & AULTC & Event & c-index & AULTC \\
\midrule
\textbf{LLM-MLP head} &&&& &&\\
\quad DS-L3.3 70B & 0.045 & 0.467& 0.803 & 0.602 & & \\
\quad L3.3 70B   & 0.066 & 0.463 & 0.809 & 0.614 & & \\
\quad DS-L3.1 8B & & & & & & \\
\quad L3.1 8B & & & & & & \\
\textbf{BERT-MLP head} &&&& &&\\
\quad BERT & 0.127 & 0.606 & 0.891 & \textcolor{red}{0.5} & 0.405 & \textcolor{red}{0.5}\\
\quad RoBERTa & 0.132 & 0.523 & 0.861 & \textcolor{red}{0.5} & 0.346 & \textcolor{red}{0.5}\\
\quad DeBERTa-small  & 0.243 & 0.601 & 0.894 & 0.56 & 0.392 & 0.517\\
%\quad DeBERTa-large   &&&& &&\\
\quad ModernBERT-base & 0.19 & 0.619 & 0.902 & 0.574 & 0.379 & 0.541\\
\quad ModernBERT-large & 0.206 & 0.610 & 0.894 & 0.541 & 0.378 & 0.498\\
\bottomrule
\end{tabular}
\end{table*}

